On the Minimal Knowledge Required for Solving Stellar Consensus

Byzantine Consensus is fundamental for building consistent and fault-tolerant distributed systems. In traditional quorum-based consensus protocols, quorums are defined using globally known assumptions shared among all participants. Motivated by decentralized applications on open networks, the Stellar blockchain relaxes these global assumptions by allowing each participant to define its quorums using local information. A similar model called Consensus with Unknown Participants (CUP) studies the minimal knowledge required to solve consensus in ad-hoc networks where each participant knows only a subset of other participants of the system. We prove that Stellar cannot solve consensus using the initial knowledge provided to participants in the CUP model, even though CUP can. We propose an oracle called sink detector that augments this knowledge, enabling Stellar participants to solve consensus.

==> links-to-figures.tex <==
where-consensus-can-be-solved:
    https://www.mathcha.io/editor/8XLKdcz2FrMfGzh090qjJTmp4L63i1drQ0BiWmPkGE

example stellar:
    https://www.mathcha.io/editor/rZD6NCM1fL0S4gtdYrDOdSqzWg8oHp96J3fOD7OPz

proof: 
    https://www.mathcha.io/editor/YXyKMFELidxIj6UK782OlHdWzkoEtzx83p2S4z071k

example cup:
    https://www.mathcha.io/editor/mPDYWtoBi8nsGwh0Ez7QwUxvKezrC3J0B9Df5NkX5m

correctness proof:
    https://www.mathcha.io/editor/r9O89FM1fL0S4gtGX5lr7H4Mj5QnuBr6WBLTLD6p4V
